Classifying Latent Infection States in Complex Networks

Algorithms for identifying the infection states of nodes in a network are crucial for understanding and containing infections. Often, however, only a relatively small set of nodes have a known infection state. Moreover, the length of time that each node has been infected is also unknown. This missing data -- infection state of most nodes and infection time of the unobserved infected nodes -- poses a challenge to the study of real-world cascades. In this work, we develop techniques to identify the latent infected nodes in the presence of missing infection time-and-state data. Based on the likely epidemic paths predicted by the simple susceptible-infected epidemic model, we propose a measure (Infection Betweenness) for uncovering these unknown infection states. Our experimental results using machine learning algorithms show that Infection Betweenness is the most effective feature for identifying latent infected nodes.

==> problemstatement.tex <==
\section{Problem Statements}
\subsection{Spreading Model}
We consider a network model of an undirected graph $G(V, E)$, where $V$ is a set of nodes and $E$ is a set of edges that represent the connections between the nodes. A malfunction (epidemic) can be propagated through paths that consist of available edges. Of epidemic spreading models that have been suggested, we focus on the SI model. The infection propagation time between nodes follows  an exponential distribution with the spreading rate $\lambda$ at which each susceptible node is infected from an infected neighbor node during one time slot.

\subsection{The Problem}
We suppose that there are $l$ observed nodes $L = \{(x_1, y_1)$, ..., $(x_l, y_l)\}$ and $u$ unobserved nodes $U =\{x_{l+1}$ ..., $x_{l+u}\}$; $l$ is typically much smaller than $u$, and $y$ has a value of $\{0, 1\}$ where $0$ and $1$ represent susceptible and infected, respectively. Given the observed nodes $L$, our task is to assign appropriate labels to the unobserved nodes $U$. In addition to $L$, we assume that the elapsed time $t$ after an epidemic starts is available; for example, we know when a DDOS attack to a particular node is started by worm-infected nodes in computer networks. This assumption allows us to estimate the boundary of infected nodes; without $\lambda$ and $t$ we cannot restrict the number of infected nodes in networks. Figure \ref{fig:problem} illustrates our problem setting.

    \begin{figure}[!hhh]
    \centering
    \caption{The red nodes and white nodes represent infected and susceptible nodes, respectively. The nodes in shaded region are observed (labeled). Note that observed nodes need not to be in one connected component. We infer the label (status) of unobserved  nodes (dotted circles) given observed nodes.}
    \label{fig:problem}
        \includegraphics[scale=0.25]{./problem.eps}
    \end{figure}

\subsection{Relation to Semi-Supervised Learning}
Various graph-based approaches for semi-supervised learning have been proposed relying on the idea of building a graph whose nodes are data points and edges represent similarities between points. In our problem, we already have a graph structure which illustrates nodes and their connected/disconnected relationships; therefore, we can easily formulate a semi-supervised learning problem based on graphs by determining an appropriate similarity matrix that can reflect the epidemic behaviors. In the following section, we will discuss how to build the similarity (weight) matrix for our problem and how to use it for determining the status of unobserved nodes.


